Minimax Performance Limits for Multiple-Model Estimation

This article concerns the performance limits of strictly causal state estimation for linear systems with fixed, but uncertain, parameters belonging to a finite set. In particular, we provide upper and lower bounds on the smallest achievable gain from disturbances to the point-wise estimation error. The bounds rely on forward and backward Riccati recursions -- one forward recursion for each feasible model and one backward recursion for each pair of feasible models. We give simple examples where the lower and upper bounds are tight.

==> figures/problem.tex <==
\begin{tikzpicture}[node distance = 6em, line width=0.5mm, inner ysep=6pt, >=latex]
	\node[block] (state_update) {$x_{t+1} = Fx_t + w_t$};
	\coordinate[left=2em of state_update] (input) {};
	\node[block, right=2em of state_update] (H) {$H$};
	\node[sumcircle, right=2em of H] (sum1) {};
	\coordinate[above=2em of sum1] (noise) {};
	\node[block, right =2em of sum1] (mu) {$\mu$};
	\node[block, right=2em of mu] (z) {$z^{-1}$};
	\node[sumcircle, right=2em of z] (sum2) {};
	\coordinate[right=2em of sum2] (output) {};

	\draw[->] (input) -- node[above] {$w$} (state_update);
	\draw[->] (state_update) -- node[above] (x) {$x$} (H);
	\draw[->] (x) -- ([yshift=-3em]x.south) -| node[pos=0.9, left] {$-$} (sum2);
	\draw[->] (noise) -- node[right] {$v$} (sum1);
	\draw[->] (H) -- (sum1);
	\draw[->] (sum1) -- node[above] {$y$} (mu);
	\draw[->] (mu) -- node[above] {$\hat x$} (z);
	\draw[->] (z) -- (sum2);
	\draw[->] (sum2) -- node[above] {$\tilde x$} (output);
\end{tikzpicture}

